Designing Loving-Kindness Meditation in Virtual Reality for Long-Distance Romantic Relationships

Loving-kindness meditation (LKM) is used in clinical psychology for couples' relationship therapy, but physical isolation can make the relationship more strained and inaccessible to LKM. Virtual reality (VR) can provide immersive LKM activities for long-distance couples. However, no suitable commercial VR applications for couples exist to engage in LKM activities of long-distance. This paper organized a series of workshops with couples to build a prototype of a couple-preferred LKM app. Through analysis of participants' design works and semi-structured interviews, we derived design considerations for such VR apps and created a prototype for couples to experience. We conducted a study with couples to understand their experiences of performing LKM using the VR prototype and a traditional video conferencing tool. Results show that LKM session utilizing both tools has a positive effect on the intimate relationship and the VR prototype is a more preferable tool for long-term use. We believe our experience can inform future researchers.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> Source/1-introduction.tex <==
\section{Introduction}

Many people encounter the situation of a long-distance relationship because of career or academic opportunities and unexpected events, e.g., social and traveling restrictions during the pandemic. Isolating from the romantic partner tends to intensify the intimate relationship because of the lack of physical contact, insufficient sensed presence, the latency of synchronization of information and compassion, and so on ~\cite{kjeldskov2004using, greenberg2009awareness, bales2011couplevibe}. Compared to traditional connection approaches (e.g., phone calls, videos), researchers also came up with many creative ones, such as gloves, cups, and pillows ~\cite{singhal2017flex, guo2019if, li2018review}. However, the experience delivered by these approaches is an implicit communication as users only interact with some object used in a particular scenario in daily life. In contrast, social VR can provide a more immersive social experience for people in a long-distance relationship and improve the sensed social presence by providing the online experience of many real-life activities, such as chat, meditation, meetings, and church activities ~\cite{mcveigh2019shaping, mcveigh2018s,maloney2021social}. 

%loving-kindness meditation has not yet received enough attention among these activities yet. However, loving-kindness meditation is an effective intervention in clinical psychology to cultivate compassion and empathy, which positively correlated with the experience of romantic relationships ~\cite{atkinson2013mindfulness, gencc2021transforming, cunningham2012loving, atkinson2013mindfulness, mapp2013relationship}. Current studies have already demonstrated the feasibility and strengths of creating interactive meditation experiences with multi-media technology ~\cite{vacca2016designing, Mah2020, Mah2020RitualInteraction}. 

%However, existing VR meditation prototype studies mainly focus on individual meditation experiences. The very limited cases make it hard to conclude general design guidance and suggestions for romantic relationship users' meditation VR prototype in terms of virtual environments, interaction objects, privacy issues, etc. To fill this research void, we adopted a participatory design process to collect qualitative data to explore the design guidelines. 

In addition to real-life activities, \textit{loving-kindness meditation} has been shown to be an effective intervention in clinical psychology to cultivate compassion and empathy, which positively correlate with the experience of romantic relationships ~\cite{atkinson2013mindfulness, gencc2021transforming, cunningham2012loving, mapp2013relationship}.  
Although not focusing on romantic relationship users, interactive meditation with multimedia technology has been shown to be able to cultivate compassion and empathy ~\cite{vacca2016designing, Mah2020, Mah2020RitualInteraction}. While inspirational, these prior work did not focus on VR, which can provide more immersive environments for meditation. Moreover, current VR meditation applications mostly focus on individual experiences than pairs ~\cite{roo2017inner, kosunen2016relaworld, patibanda2017life, prpa2018attending, yildirim2020efficacy} . 
Inspired by these pioneering work, we hypothesize that interactive loving-kindness meditation in VR might provide new opportunities to promote healthy long-distance romantic relationship.
However, it remains an open question of how best to design VR elements, such as virtual environments and interactive objects, to support loving-kindness meditation experience between romantic partners.

To answer the research question, we adopted a participatory design process by conducting design workshops with 7 pairs of participants who were in romantic relationships. During the workshop, the pair first practiced loving-kindness meditation, experienced different meditation virtual environments as well as physiological signals collection technology, and then designed VR environments and elements that they would love to have when performing loving-kindness meditation together. Finally, they were interviewed about their experiences and the rationales of their designs. We analyzed the rich set of data gathered from the workshops and derived key design considerations. To be more specific, participants seek security and exploration in environment settings; regarding to avatars, participants preferred avatars that can capture their realistic appearances or at least some key characteristics of their look; all participants mentioned an inserted audio communication was required, and other frequently mentioned intimate interactions were hand holding, hugging, head touching, kissing, etc.; participants showed less desire to display the visualization of their bio-signals, less interest to interact with non-creature objects in the environment such as water, stones, or plants, and less demand on privacy. 

Informed by the design considerations derived from the design workshops, we further designed and implemented a VR prototype to further explore how romantic partners would use it to perform loving-kindness meditation and whether it is feasible for the prototype to introduce positive experiences to their meditation. We re-invited two couples to experience the prototype for six sessions and assessed their experiences of doing loving-kindness meditation with the prototype using psychological instruments, skin conductance, and qualitative feedback. Results show that it is feasible to do loving-kindness meditation via VR for users in a long-distance relationship and participants showed high interest in this approach; however, there are special design principles for an intimacy relationship social meditation VR prototype, which are different from individualized meditation VR prototypes. 

In sum, we make the following contributions:

\begin{itemize}
\item We derived design considerations through participatory design workshops for creating loving-kindness meditation experiences in VR for romantic partners.
\item We showed the feasibility of providing positive experiences to romantic partners by understanding how they used a loving-kindness meditation VR prototype designed and implemented based on the design considerations. 
 
\end{itemize}



==> Source/2-related-work.tex <==
\section{Background and Related Work}
\subsection{Long Distance Relationship}
% With the globalization of the job market, the advancement of traveling technologies, and the improvement of communication technologies, the number of long-distance relationship cases keeps increasing~\cite{Wei-Chi2020, Hassenzahl2012,Merolla2010}.
The number of long-distance relationship instances continues to rise due to the globalization of the employment market, the development of travel technologies, and the enhancement of communication technology~\cite{Wei-Chi2020, Hassenzahl2012,Merolla2010}. 
Especially during the COVID-19 pandemic, people unavoidably tend to fall into social isolation due to unexpected social and traveling restrictions and apart from their romantic partners~\cite{Fego2021, aspikom718, maiti2020marital}. 
Long-distance relationships always face obstacles, such as an inadequate sensation of each other's presence~\cite{kjeldskov2004using}, 
% The maintenance of long-distance relationship meet inevitable challenges, such as insufficient sense of each other's presence~\cite{kjeldskov2004using}, 
% difficulties in synchronizing individual emotional status and expressing compassion ~\cite{greenberg2009awareness}, 
difficulties in coordinating emotional states and conveying empathy~\cite{greenberg2009awareness},
lack of physical contact~\cite{bales2011couplevibe}, etc. 
To address these challenges, HCI scholars have adopted various technologies to assist in maintaining a long-distance relationships. Many solutions are designed to enhance communication and interaction between partners based on personal electronic devices like smartphones (e.g., video, instant messages, and a chat robot)~\cite{guo2019if, li2018review, tang2017collaboration, zheng2021pocketbot}, while some other solutions created more physical feelings and emotional relatedness with specific devices (e.g., gloves, cups, pillow and bed) ~\cite{singhal2017flex, chung2006lover, dodge1997bed}. 

\subsection{Social VR}
Although the aforementioned solutions effectively achieve their design objectives, the interaction with the user's partners is not immersive enough. Compared to the solutions on conventional mobile devices, social VR can deliver a more immersive experience of real-life social activities and events through the low-latency, high-resolution 3D environments presented by head-mounted displays or other relevant displays~\cite{mcveigh2019shaping, mcveigh2018s}. For example, Zamanifard and Freeman reveal that users in a long-distance relationship can feel together by replicating real-life activities~\cite{zamanifard2019togetherness}. Emma Yann Zhang and Adrian David Cheok's work created kissing experiences in VR~\cite{zhang2021turing}. Rukangu et al. proposed a customized virtual family room to mitigate the impact of physical separation among family members~\cite{rukangu2020virtual}. 
AltspaceVR is a well-known commercial social VR platform that enables users to engage in a variety of social activities and events,
% AltspaceVR, a popular commercial social VR platform, allows users to proceed with various social activities and events, 
such as open mic night, comedy, meditation, yoga, and VR church~\cite{maloney2021social}. 

\subsection{Loving and Kindness Meditation}
Among the social VR activities or events designed for users in a long-distance relationship, loving and kindness meditation are less discussed. However, more efforts could be put in. Grounding in Buddhism, loving-kindness meditation is a particular type of meditation aiming at cultivating kind attitudes towards oneself and others, including romantic partners, family members, friends, strangers, or even any creatures in the world~\cite{zeng2015effect}. In psychology, loving and kindness meditation are introduced into couple relationship therapy as it can cultivate compassion, and empathy~\cite{atkinson2013mindfulness, gencc2021transforming, cunningham2012loving}. Some studies also indicated that compassion and empathy intervention positively correlate with the satisfaction of long-distance romantic relationships~\cite{atkinson2013mindfulness, mapp2013relationship}.

\subsection{Multi-users VR meditation}
Currently, the amount of loving and kindness meditation VR prototypes for people in a romantic or long-distance relationship is very limited. In the DYNECOM prototype~\cite{salminen2019evoking}, users' EEG signals and respiration rhythm are visualized beside their avatars in the virtual environments while doing loving and kindness meditation. Even though the visualization of biosignals improves the sense social presence, the prototype aims at conventional loving and kindness meditation. It is not tailored for couples or people in a romantic relationship. For example, the avatar is gender neutral statue to avoid any identity information. The visualization of bio-signals improves the sense of social presence. The JeL~\cite{desnoyers2019jel} presents underwater scenes: two jellyfish as the avatars and one interactive virtual coral. The jellyfish's floating is a visual guide for users to do mindfulness breathing exercises, 
and the coral's growing offers a creative interaction for two users to maintain synchronized respiration. The interaction strengthens the bond between two users, however, this prototype is not intended for those in romantic relationships.
%and the coral's growth is a creative interaction for users to keep respiration synchronization. The interaction enhances the connection between two users, but this prototype does not target people in romantic relationships. 

% Existing studies are inspiring, whereas less can be summarized about the design principles of the virtual environments, interactive objects, avatars representation, etc., since the limited amount of studies and heterogeneity of these designs. There is much space 
% for exploring the design principles of VR meditation prototypes for users in a long-distance relationships. 
Existing studies are enlightening, but it is more difficult to describe the design principles of virtual worlds, interactive items, avatars, etc., due to the scarcity of research and heterogeneity of these designs. There is a great deal of room for investigating the design concepts of VR meditation prototypes for individuals in long-distance relationships. 
Therefore, our study adopted a user workshop design process to explore. 


==> Source/3-method.tex <==
\section{Method}

% To address the question of how to create the virtual reality-based shared meditation environment desired by the target users based on their preferences, we divided the study into four phases.
%The research was split into four parts to answer the issue of how to develop the VR-based LKM environment required by the target users of romantic relationships.
% First, we planned four participatory workshops for couples to evaluate how virtual reality can be used for meditation and improve intimacy for couples in a long-distance situation. 
%First, we organized four participatory workshops for couples to assess how VR can be utilized for LKM and to enhance long-distance couples' connection and intimacy. 
%Second, following workshop implementation, we conducted a detailed analysis of how participants understood and organized themselves when creating VR scenes and designing VR interactions. 
%Second, following the workshop implementation, we did a comprehensive examination of how participants understood and structured themselves while planning VR interactions in distal and constructing VR scenarios. 
% Next, we summarized the design elements of the workshop and used them as a reference to create a VR remote couple meditation prototype. 
%Next, we summarized the workshop's design concepts and applied them to construct a VR LKM prototype designated for remote couples.
%Finally, we again invited two couples who had participated in the workshop to experience our prototype, evaluate its feasibility, and discuss how the workshop approach could be used to tailor a VR remote meditation application for couples. 
%Finally, we invited 8 couples to test our prototype, assess its feasibility, and explore how the workshop technique may be utilized to customize a VR remote LKM application for couples.
%Below, we provide descriptions of the participants and then detail the structure of the participatory design workshop that included this study, as well as the methods used to analyze the workshop data.

%Due to the scarcity of research and heterogeneity of designs, it is difficult to refer to design implications about virtual environments, interaction objects, avatars, etc. To address the question, 
To answer our RQ, we first conducted participatory design workshops with couples in long-distance relationships to understand how they would want VR to be designed for them to perform LKM better. From the multiple sources of data gathered from the workshops, we derived design considerations and designed a VR app accordingly. We then invited another group of couples in long-distance relationships to perform LKM with the prototype and a traditional VC tool. We derived insights into the effects of the VR prototype on their LKM experiences and ways to improve VR LKM experiences further.  

% which aims to investigate user-centred design implications (section XXX). Couples experienced the LKM session, diverse VR environments referring to existing studies and physiological signals detection technology in the workshop. Next, couples expressed their expectations for a VR meditation application supporting LKM on canvas. At last, a semi-structured interview was conducted for each pair to investigate the reasons for their designs. Multi-types of qualitative data, including couples’ drawings, interview scripts, and other observed behaviour during the workshop, were analyzed to investigate design implications for the prototype design. The second phase is prototype designing, implementation and evaluation (section XXX). Based on the analysis from the first phase, we made decisions about VR environments, avatars, interaction methods, etc., and implemented the prototype. Then, we invited another group of participants to experience the prototype. Finally, we adopted psychological instruments to evaluate participants’ responses to the prototype.  


%\subsection{Participants}
%Our participants were recruited by advertising on social networks, and all participants were students from two local universities. We required that participants %be unmarried couples 
%who had either some experience with meditation, or an interest in meditation, or an interest in design techniques, to participate together. It is preferable that couples have experience in a long distance relationship.

%9 couples registered for the workshop, of which 2 were unable to attend due to unavailability of time and partner's absence from the city, and 7 couples (7 female, 7 male, 14 in total) ended up participating in the workshop. Participants’ ages ranged from 22 to 27 years (M = 23.64, SD = 1.39). All participants are from Eastern cultural backgrounds. All couples experienced long-distance situations, and 4 couples had long-term long-distance experiences (>1 year). Regarding meditation knowledge and experience, most participants are novice levels, and only 1 couple reported having meditation experiences with their partner. A small number of participants had experience with VR (n=4). All participants personally signed an informed consent form before the workshop, and each participant was compensated \$20 at the end of the workshop. Table~\ref{tab:participants} shows the codes and other details for each pair of participants.

% \begin{table}[h]
%   \caption{Participant demographics (self-reported during recruitment)}
%     \renewcommand\arraystretch{1.20}
%   \label{tab:participants}
%  \resizebox{1\linewidth}{!}{ 
%   \begin{tabular}{p{40pt}p{40pt}p{80pt}p{80pt}|p{40pt}p{40pt}p{80pt}p{80pt}}
%     \toprule
%     Code & Age & Relationship length &  Separation duration & Code & Age & Relationship length &  Separation duration \\
%     \hline
%     \rowcolor{gray!8} 
%     $C1_F$ & 24 & 6 years & 5 years & $C5_F$ & 23 & 4 years & 3 years\\
%     \rowcolor{gray!8} 
%     $C1_M$ & 24 &  & & $C5_M$ & 23 & &  \\
%     $C2_F$ & 24 & 4 years & 2 years & $C6_F$ & 22 & 2 years & <1 year \\
%     $C2_M$ & 27 &  & & $C6_M$ & 22 &  & \\
%     \rowcolor{gray!8}
%     $C3_F$ & 24 & 2 years & 1 year & $C7_F$ & 23 & 2 years & 2 months\\
%     \rowcolor{gray!8}
%     $C3_M$ & 25 & & & $C7_M$ & 25 & & \\
%     $C4_F$ & 22 & 1 year & 1 week & & & &\\
%     $C4_M$ & 23 &  & & & & & \\
%     \bottomrule
% \end{tabular}}
% \end{table}

%\subsection{Participatory workshop}

%The study was conducted in an empty office area of a local university. The location was chosen because 1) it provided enough space for participants to be placed in two empty conference rooms separated by walls to create a sense of remoteness, 2) the views were great and participants could experience the sea and hills from floor-to-ceiling windows, and 3) it was quiet and undisturbed. The two co-first authors were responsible for planning and implementing the four workshops. After each workshop, our team held a meeting with all authors to discuss the findings of the previous workshop, plan for the next workshop, and brainstorm for the development of the prototype application.

%Except for the first workshop where only one couple attended, the next three workshops were attended by two couples (4 people in total) together. Our study considered the first workshop as a pilot study, and some findings from that allowed us to adjust the setting of the subsequent three workshops and the preparation of workshop materials (which will be discussed in detail in Table~\ref{tab:materials}), with the setting of the latter three workshops remaining consistent.

% \begin{table}[h]
%   \caption{List of stationery materials used in the workshop}
%     \renewcommand\arraystretch{1.20}
%   \label{tab:materials}
%  \resizebox{.7\linewidth}{!}{ 
%   \begin{tabular}{p{120pt}p{40pt}|p{120pt}p{40pt}}
%     \toprule
%     Name of stationery & Number & Name of stationery & Number \\
%     \hline
%     Scissor & 3 & A3-size white sketch paper & 20\\
%     12-color watercolor pencils & 1 & 24-color chalk & 1 \\
%     Transparent adhesive & 3 & Glue stick & 3 \\
%     Sticky Notes & 2 & A4-size Colored cardstock & 40 \\
%     Double-ended black marker & 4 & Pencils & 3\\
%     Eraser & 3 & & \\
%     \bottomrule
% \end{tabular}}
% \end{table}

%\subsection{Data collection and analysis}

%Participants were videotaped throughout the workshop with their permission using tripods and smartphone cameras in order to capture all the participants' collaboration scenarios. During the workshop, we conducted semi-structured interviews with the participants and we recorded the interviews with participants' permission. After interview, all recordings were transcribed into scripts and imported to Nvivo\footnote{\url{https://www.qsrinternational.com/nvivo-qualitative-data-analysis-software/home}} to proceed an thematic analysis. The themes were mainly referred to several works and adapted to our situation~\cite{wienrich2020mind, dollinger2021challenges, terzimehic2019review}. In the work of Wienrich et al., 
%VR is defined as %they defined VR as 
%\emph{virtual environment, virtual interactive
%objects, virtual others, and virtual self-representation}~\cite{wienrich2020mind}. 
%We adapted the themes as \emph{virtual environment, avatars (virtual others and virtual self-representation), interaction in VR (virtual interactive objects)} and bio-signals detection. In addition, a \emph{privacy} theme and a \emph{design process} theme was added since intimacy social behaviors were included~\cite{maloney2021social}. The coding process was proceeded separately by two researchers, and any differences were fully discussed until both researchers reached consent. Besides interview data, other qualitative data were collected, such as workshop photographs, participants' design work, and post-workshop meeting notes.

%\subsection{Equipment and materials}

%Since the vast majority of the participants had novice experience with meditation, and only a small number of them had VR experiences. We used a MacBook Air M1 to play guided meditation audio for about 10 minutes. Since there are very limited works for users in romantic relationships to do LKM, we created the customized meditation guidance audio. First, we wrote a customized guidance script referring to LKM literature ~\cite{sujiva2009meditation, seppala2009loving, vacca2016designing}. Then we adopted Microsoft Azure ~\cite{MicrosoftAzure} to proceed with text-to-speech transformation to create a constant speech experience for all participants instead of reading by experimenters.The computer agent name we selected is Xiaoqiu (Neural), the speaking style was set to General, the speech speed was set to 0.74, and the pitch was set to 1.00.
%Then, in a video/audio editing software named BeeCut~\cite{BeeCut}, we combined yoga non-script background music with the generated speech. 
%Then, we added yoga non-script background music with the transformed speech in a Video/audio editing software named BeeCut ~\cite{BeeCut}. 
%We used Unity to prepare the Virtual Reality environments and two Oculus Quest 2 to present these environments to participants. The environments provided to participants were inspired by existing multi-media meditation studies. We finally ended up with 11 environments based on existing studies ~\cite{roo2017inner, patibanda2017life, desnoyers2019jel, feinberg2022zenvr}. Since many of the previous experiments on the topic of VR and meditation involved physiological data~\cite{roo2017inner,patibanda2017life,stepanova2020jel,mevleviouglu2021visual}, our workshop also allowed participants to experience the measurement of physiological data. As such, we employed %using 
%the ProComp5 Infiniti basic package and the skin conductance sensor(SC-Flex/Pro) ~\cite{ThoughtTechnology} to measure the skin conductance to provide cues for participants. The measured data were analyzed in Matlab. The prototype design used the same VR equipment as the workshop.



==> Source/5-results.tex <==
\section{Results}
This section presents the results according to a thematic analysis according to %result of 
the rich set of data from workshop sessions. The analysis focused on meditation virtual environments, avatars, interaction in VR, bio-signals detection and visualization, design process, and privacy.

\subsection{Meditation Virtual Environments}
% To investigate users' preference on meditation virtual environment, we first presented them 11 virtual environments, inspired by prior VR meditation studies ~\cite{} and then invited them to rank those environments based on their favorability ; then in the design process, we offered various materials for them to design their own virtual environments for a VR meditation prototype and then conducted semi-structured interview asking their design rationales. This section elaborated the result of user' preferable virtual environments rating and findings of interview on design output. 

%Although the details in each participant's feedback in the interview, ranking of environments favorability, design drawings, etc. were diverse due to individual preferences, some common characteristics could be concluded. First, natural elements were widely mentioned; Second, participants showed an obvious requirement for a sense of security when designing the setting of the scene; Third, multiple environments are preferred other than only one environment; Fourth, one of the environments was expected to provide more sense of security, more space for individualization, and longer experience; Lastly, an environment that changes spontaneously according to some rules is better than one that remains unchanged, for example, day and night.





\subsubsection{Analysis of qualitative data}
 

% Although the details in the interview, design, videos and workshop notes of each participant were diverse due to individual preferences, some common characteristics could be concluded. First, users have a preference for settings that can provide a sense of security and a relatively rich visual array; second, users express the desire to explore other diverse scenes with having a safe place as the "base"; third, users expressed the idea of experiencing a dynamic scene, specifically, time change and diurnal shift. (I will edit this paragraph later)
\par
\textbf{Nature.} 
All participants drew natural elements in their design (see Figure \ref{fig:examples}), such as grass, flowers, trees, rivers, etc. 
%In their explanation, they indicated the desire to contact nature and get away from stressed daily work scenarios such as computers, offices, and highways to relax. This was constant with the findings in environments favorability ranking that environments 1 to 8 received better feedback than 9 to 11.  In addition, five pairs drew animals in the designed scenes, such as birds, cats, dogs, fishes, etc. Participants' preference for animals was also corresponding with the findings in environments favorability ranking (1 vs. 2 and 3 vs. 4). 
In their explanation, they expressed a desire to reconnect with nature and escape from stressful work environments such as computers, offices, and motorways in order to unwind. In addition, five couples drew animals, such as birds, cats, dogs, fish, etc. in the planned scenarios. The participants' preferences for animals were also in line with how attractive they thought the settings were (1 vs. 2 and 3 vs. 4).

%

%Consistent with the VR sorting results, the six couples' designs involved animal elements. The secure place gives couples a sense of warmth and security, but animals in the wild is a reflection of insecurity, so no couples want to appear in their ``secure base'' wild animals, even if they look very tame, such as deer. But they prefer to have cats and dogs and other pets in their homes, and want to be able to interact with pets. Other widely mentioned visual elements contained natural elements such as plants, rivers, garden, oceans, etc. 

\begin{figure}[h]
  \centering
  \includegraphics[width=1\linewidth]{Figures/examples.png}
  \caption{Four examples of participants' drawings to illustrate the meditation scene in their minds. a) The avatar representing the couple is sitting on a stone bridge with a kitten lying next to them, and the sketch shows the different scenes they wish to experience; b) participants drew imaginary houses and gardens of their own; c) participants drew their own houses and a garden with a large lavender field, with a double swing for them to lie shoulder-to-shoulder; d) the participants' avatars sat shoulder-to-shoulder in the spaceship, and they took the spaceship to the four scenes drawn on the sketch and sketched with cats, which they wished to have with them.}
  \Description{Four examples of participants' drawings to illustrate the meditation scene in their minds. a) The avatar representing the couple is sitting (confirmed with the participants, although the cartoon stickers they casually chose to look like standing) on a stone bridge with a kitten lying next to them, and the four corners of the sketch show the different scenes of the four they wish to experience, each with natural elements; b) participants drew imaginary houses and gardens of their own, with sofas and floor-to-ceiling windows in their homes and bellflowers, mailboxes and garages in their gardens. Participants were not good at drawing and labelled many text explanations in their sketches; c) participants drew their own houses and a garden with a large lavender field, with a double swing for them to lie shoulder-to-shoulder to view the lavender field; d) the participants' avatars sat shoulder-to-shoulder in the spaceship, and they took the spaceship to the four scenes drawn on the sketch: home, underwater, starry sky and natural environment, and sketched with cats, which they wished to have with them.}
  \label{fig:examples}
\end{figure}


\begin{quote}
    \textit{``... There is a cat sleeping on the windowsill, I want to have cute animals in the house, instead a dog I would prefer a cat, in the real world I do not yet have a cat ...'' - $C1_F$}
\end{quote}


\textbf{Sense of security.} In terms of the settings or layout of the environments, all participants designed elements and spaces that provide them with different degrees of safeguarding and support., ranging from a bridge (Figure~\ref{fig:examples}~a)), an airship (Figure~\ref{fig:examples}~d)), a house (Figure~\ref{fig:examples}~b) \& d)). 
%They said they hope to be on a firm foundation in a safe setting, where they could sit, stand, or lie down, to view the rest of the environment. 
They expressed a desire to be seated, standing, or lying down on a stable platform in a secure location from which they may see the rest of the surrounding environment.

\begin{quote}
    %\textit{``I originally wanted to draw a big fence to divide us from the animals but so difficult to draw, anyway, I drew a bridge so we can stand on the bridge. Other animals are at the surrounding of the bridge. And, yes, yes, the bridge is sort of artificial architecture and it is a relatively safe place to stay.'' - $C2_M$}
    
    \textit{``I want to be in my own house with my boyfriend, two floors, wooden spire, a small but cozy second-floor loft where we can lie down and relax together, with moonlight coming in through the windows... '' - $C5_F$}
 
\end{quote}

%The pursuit for sense of security also reflected in the environments favorability ranking 
%The pursuit of a sense of security is also reflected in the ranking of the environment's favorability (Figure \ref{fig:Ranking of Environmental Favorability}). For example, the realistic animals in the dense deciduous woods reminded them of wild animals and caused insecurity, so that the environment received a relatively lower ranking (2 vs. 4 in Figure \ref{fig:Ranking of Environmental Favorability}). 
%For another instance, the dense deciduous woods, with dense woods blocking participants sights, received relatively lower ranking comparing with woods with river, with more permeable space configuration allowing participants to see far away (1 vs. 3 in Figure \ref{fig:Ranking of Environmental Favorability})
%As mentioned, the dense deciduous woods, with dense woods blocking participants' sights, received a relatively lower ranking compared with woods with a river, with a more permeable space configuration allowing participants to see far away (1 vs. 3 in Figure \ref{fig:Ranking of Environmental Favorability}).


%\textbf{Multiple environments.} All participants implied that they would like to leverage different environments in a meditation VR app. Some participants wanted to view the scenes from different perspectives, for example, to appreciate the garden view from inside and outside the house (Figure~\ref{fig:examples}~b) \& c)). Some other participants wanted to directly switch among different environments, which could be some special places where they have shared memories or some interesting destinations on their travel plan (Figure~\ref{fig:examples}~a) \& d)). To summarize, they provide two reasons. First, they said only one scene for meditation might be monotonous and tedious as it is a high-frequency and long-time exercise. Second, some participants emphasized that they needed a particular scene as the stimuli and buffering allowed them to calm down gradually before formally starting meditation. 

%This corresponds to the forest scene scored very low when choosing a preferred VR scene before. Several participants who scored the forest scene the lowest indicated that the forest would make him feel very insecure, which is consistent with the XXX study. 

%\begin{quote}
    %\textit{``I would like to have a house and garden of our own...we would like to walk out of the house together and see the garden. A garden with a swing and a big field of lavender... I really like lavender and it would be nice to be able to smell it!'' - $C3_F$,$C3_M$}
    
    %\textit{``The room walks out to a yard with a botanical garden, a small garden, a garden with lily of the valley, which I like, and my boyfriend wants a mailbox and a garage, hmmm... this is very life-like, the kind of home we want to have in reality.'' - $C5_F$}
    
%    \textit{``We can go to anywhere to meditate in this open world, for example we are in a ship or an airship and we just lie in it and see the views outside the window, this side might be nature, that side might be the ocean, and inside the airship it just like our home.'' - $C4_M$}
    
%\end{quote}

 \textbf{Personalized spaces.} Reflected by the design drawings and interviews, participants implied that they would like to stick to one environment as the base, which means maintaining long-term and adding personalized items gradually to create shared memories.  

\begin{quote}
    %\textit{``We can enjoy a carefree life inside this travelling machine and then drive it to various places, for example, go to an island.'' - $C7_M$}
    
    \textit{``The bedroom could be a more private space that contains more activities. We can also arrange this space together. For example, we can decorate the same room online. There would be some furniture models, or maybe, wallpapers, to select, so that we can decorate together.'' - $C7_F$}

    
\end{quote}

\textbf{Dynamic environment.} Half of the participants proposed the idea that they want to experience a dynamic environment, for example, time change and day/night shifts, so that they can experience different scenery such as sunset at dusk, early morning sunrise, and the starry night sky. 
%They expected the attributes that can be changed were corresponding with real life but they can have the right to manipulate these attributes so that they can experience difference scenery that they cannot in real life. 
They expected the attributes that could be changed to correspond with real life, but they can have the right to manipulate these attributes so that they can experience different scenery that they cannot experience in real life.

\begin{quote}
    %\textit{``but this change don't need to be exactly the same as reality, it could be 90 minutes a day in VR, yes, yes...and when you login in this environment, you may just encounter a scenery of rain'' - $C1_M$}
    
    \textit{``something that could be kept consistency with the reality, for example, Christmas and Spring Festival, when you login, yes, this environment is in the atmosphere of festivals.'' - $C2_F$}

\end{quote}


%This need for "base", multiple scenes and pet scenes was beyond our expectations, as none of the 11 scenes the participants experienced prior to the design met these needs, but they were surprisingly consistent in the couple's design.

\subsubsection{Ranking of VR Environments Favorability}
%In the VR scenes experience session, participants were invited to rank the environments based on their favorability with an 11-Point Likert Scale (1 = the least favourite, 11 = the most favourite). Therefore, we present here some descriptive statistics. The 11-point Likert Scale is employed due to ranking the 11 scenes from the most preferred to the least. 

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{Figures/ratings_0911.pdf}
    \caption{Ranking of Environments Favorability. Participants were invited to rank the environments based on their favorability with a 11-Point Likert Scale (1 = the least favorite, 11 = the most favorite). The Underwater environment (7) has the highest mean value; the Calm Beach environment (6) has the lowest mean value.}
    \Description{Ranking of Environments Favorability. Participants were invited to rank the environments based on their favorability with a 11-Point Likert Scale (1 = the least favorite, 11 = the most favorite). The Underwater environment (7) has the highest mean values; the Calm Beach environment (6) has the lowest.}
    \label{fig:Ranking of Environmental Favorability}
\end{figure}

As shown in Figure \ref{fig:Ranking of Environmental Favorability}, five natural environments (1, 2, 5, 7, 8) received relatively better evaluation compared with the non-natural elements environments(9, 10, 11). 

Interestingly, three natural environments (3, 4, 6) received relatively lower favourability. Participants indicated that the impermeable space in dense deciduous woods (3, 4) made them feel insecure. Participants ($C5_F$, $C5_M$) said the beach scene was boring and monotonous at first sight, but there seemed to be some unknown threats behind the calm. This finding was consistent with the previous results that people have a preference for nature and demand for security simultaneously. 

%Additionally, dense Deciduous woods (3) that blocked participants' sight also induced some feel of insecurity, resulting in more negative feedback. 
%Dense deciduous woods (3) made it hard for people to see and made them feel unsafe, leading to more negative feedback.
%One participant said that it seems that something would rush out from the dense woods. Correspondingly, the Woods with river (1) received a relatively better ranking with more permeable space allowing participants to see further away. 
%According to one participant ($C2_F$), it seemed that something would rush out of the dense woods. Similarly, the Woods with river (1) received a relatively higher ranking due to its more permeable space, which allows participants to see further away.

%However, the feedback is more heterogeneous for non-wood natural environments (5, 6, 7, 8). 
%The Bamboo forest (5) received a relatively higher evaluation with the reasons that the scene and space was simple but an atmosphere of tranquility was sensed; whereas, the Calm beach (6) was ranked as a relatively low-favorability. 
%The Bamboo forest (5) received a relatively higher rating because an atmosphere of tranquillity was sensed; The calm beach (6) received a relatively low rating.
%Our participants said the beach scene was boring, monotonous and nothing to see. In addition, the Underwater (7) and Luminous forest (8) were ranked differently, although both of them are environments not common in daily life. Participants indicated that the underwater is novel, fascinated and relaxed, while the luminous forest sometimes is mystery, weird and spooky resulting in a sense of insecurity. 
%Our participants ($C5_F$, $C5_M$) said the beach scene was boring and monotonous, and there was nothing to see. In addition, the Underwater (7) and Luminous forest (8) were ranked differently, although both of them are environments not common in daily life. Participants indicated that the underwater is novel, fascinating, and relaxing, while the luminous forest sometimes is mysterious, weird, and spooky, resulting in a sense of insecurity.

Environments (9, 10, 11) received a relatively lower ranking. More than half of the participants described that the colourful universe (9) made them feel weird, empty around and sometimes a little bit blurry eyes and dizzy when viewing the dynamic colourful aperture. The only two indoor scenes, namely Mystery temple (10) and Japanese wamuro (11), received the same feedback, such as depression, gray, monotonous, not open and not bright enough. In addition, the decorations, the sculpture and the reliefs on the wall contributed to the mystery and tension.  

%The 11 scenes experienced by each couple are: 1) bamboo forest; 2) natural environment; 3) forest; 4) underwater; 5) luminous forest; 6) temple; 7) Japanese room; 8) real animals; 9) cartoon animals; 10) universe; 11) beach. Overall, the underwater scene was the most liked and felt relaxed by the participants, and was the scene with the highest average score. However, one participant, who could not swim and was very afraid of water, felt that this scene made him very uncomfortable and gave this scene the lowest score. Cartoon animals had the second highest mean score, but was significantly different from multiple other scenes because it was generally liked by the participants and did not happen that someone hated it very much. 
%During the interviews, we found that participants did not have a very strong preference between cartoon animals and real animals, and many said that there was no difference between the two for them, 
%During interviews, we discovered that participants did not have a clear preference between cartoon animals and real animals, and many said that they did not see a significant difference between the two,
%which was also demonstrated in the analysis (p = 0.7).



\subsection{Avatars}
%All participants indicated a strong desire that the avatars need to well represent them, both their appearance and mental status, for providing each other presence and the sense of companion.
All participants expressed a strong desire for the avatars to accurately represent them, both physically and mentally (e.g., their appearance and mental status), in order to provide each other with presence and a sense of companionship.

All the couples' choices of avatars were a preference for human-like avatars. Only one couple accepted to become animals, plants or other objects, but they emphasized that the default setting should be a humanoid avatar. Their first preference was for avatars that closely resembled real people, but one participant expressed the following opinion about the Uncanny Valley~\cite{seyama2007uncanny} that would result if technically impossible to achieve.

\begin{quote}
    \textit{``I want my avatar to be very similar to myself, 100\% the same, with the exact same expressions and movements. So that my girlfriend can see my real appearance in VR. But you know, the current technology can not reach this, if the effect is not good, it will be very scary, is that the uncanny valley. So if the effect is not good I would rather avatar cartoonish, but even if cartoonish I want to be similar to me.'' - $C5_M$}
\end{quote}

For this technical problem, a couple proposed a ``look-alike'' solution. 

\begin{quote}
    \textit{``His avatar can not be exactly the same as him, but it needs to be alike, that is, the avatar's specific actions, reactions and expressions or clothing features will make me instantly associate with him, these characteristics are unique to him.'' - $C7_F$}
\end{quote}

%Half of the participants also mentioned that they need the avatar support them to display or express emotion status. 
Half of the participants also stated that they require the avatar to assist them in displaying or expressing their emotional status. 

%\begin{quote}
    %\textit{``There is another point is in VR I don't want to be a completely virtual person as well as my partner, I hope... for example, we can put the certain part of our face on the virtual avatar, or a real-time changing emojis on the virtual avatar, so that if any of us get angry and the other one can know it and change the real-time emojis into a cute and stupid thing to make each other laugh.'' - $C3_F$}
%\end{quote}

Additionally, participants mentioned that the initialization or setting of the avatars could be another potential interactive channel outside the meditation experience. For example, to design or choose avatars for each other.

\subsection{Interaction in VR}

The desired interaction behaviour of couples in the VR environment is a topic that deserves to be focused on, and this topic will be divided into
interaction (1) between couples; and (2) with virtual environments. %interaction between couples and interaction with the virtual environment.

\subsubsection{Interaction between couples}

All the couples preferred to sit or lie shoulder-to-shoulder in the static position relationship in VR (Figure~\ref{fig:examples}~a), b), c)\& d); a) Siting shoulder-to-shoulder on the bridge, b) Sitting on a double sofa), c) Lying shoulder to shoulder on a swing, d) Sitting Shoulder-to-shoulder view outside the spaceship), they gave the following reasons: shoulder-to-shoulder sitting feels closer and, more convenient for the interaction between the two of them, while the face-to-face approach will make them feel formal and not relaxed enough, but also that they are not close enough to each other. %feel that each other are not close enough. 
At the same time, they also said that if the scene didn't provide other options, they can also sit face-to-face, such as in the previous VR scene in the Japanese room.

Voice communication is a necessary feature. One couple mentioned that they would like to have some interaction between themselves as a transition before meditation, and depending on the design of all couples, these types of interactions could be hand-holding, hugging, head touching, and kissing. Hand-holding was the interaction mentioned by most of the couple participants.

\begin{quote}
    \textit{``I would really like to hug and hold hands with my girlfriend in a virtual environment...in real life, we would always hold hands all the time and hug a lot. I really like the feeling of hugging her, it makes me feel relaxed and warm, we are hugging together when we are just meditating. I would feel very good if we were long distance but could achieve this in a virtual environment, preferably with body heat and touch...'' - $C5_M$}
\end{quote}


Some of the interactions designed by couples will have stronger personal preferences and are highly relevant to the scene. For example, couples who like to play video games will want to add a shooting game scene in addition to the meditation scene. 
%But generally on for lying or sitting together to see, feel, and hear the elements of the scene.
However, lying or sitting together to see, feel, and hear the elements of the scene is generally acceptable. 
Many mention (n=4) the haptic sense, and some mention (n=2) the olfactory sense. 

\subsubsection{Interaction with the virtual environment}

%Couples who have designed pets in their scenes all want to be able to interact with their pets, such as petting them. 
All couples that include pets in their scenes want the ability to interact with them, such as slow petting and caressing them. 
%Beyond that, no couples mentioned wanting to interact with virtual environments such as flowers and plants. In general they thought that experiencing the scene was more important than manipulating and changing it.
%Comparing with interaction with each other, couples showed less interesting to in-depth engage with elements in the environments, for example, control the growth or a plant or control the river level. Participants tend to experience the environment more than manipulate them. Changing the time, light, seasons, etc. in the environment was the only aspect interaction that participants mentioned. However, the purpose for this overall adjusting is to experience difference scenery of an environment.  
Couples were interested in adjusting some overall environmental settings such as time, light, seasons, etc. rather than manipulating specific objects like controlling the growth and morphology of a tree. 

%Participants tend to experience the environment more than manipulate it. 
%Participants are more likely to observe and feel the environment than to alter it.
%Changing the time, light, seasons, etc. in the environment was the only aspect of interaction that participants mentioned. However, the purpose of this overall adjusting is to experience the different scenery of an environment.

\subsection{Bio-signals detection}
To our surprise, all couples showed relatively less interest in visualization or in-depth interaction of physical signals in the virtual environment. 
%However, visualization or interaction of personal physiological signals is a common feature in previous studies on meditation and VR \cite{}.
In previous studies on meditation and VR, however, it was common for people to see or interact with their own physiological signals~\cite{roo2017inner, jarvela2021augmented, desnoyers2019jel}. 
%First, participants were not inclined for the type of real-time data visualization such as a plot, bar, scatter, etc. They provided several concerns. Two pairs said they did not want affect each other if they are in anxious and stressed status, manifesting in the data visualization. Another pair expressed that the type of visualization would attract their attention to the result or outcomes, which might bring extra stress and tension. When we further asked the participants on how you would like to integrate the physiological signals detection in the VR meditation, they prefer intuitional and artful visualizations such as emoji or heart-shaped pattern. They even said that these emoji based on physiological detection could be only one of many emoji, and users could choose the one showing their real state, or others. 
First, participants were not inclined to the type of real-time data visualization such as a plot, bar, scatter, etc. They raised several concerns. Two pairs said they did not want to affect each other if they were in an anxious or stressed state, as manifested in the data visualization. Another pair expressed that the type of visualization would draw their attention to the result or outcomes, which might cause extra stress and tension. When we further asked the participants how they would like to integrate the physiological signals detection in the VR meditation, they preferred intuitional and artful visualizations such as emoji or heart-shaped patterns. They even said that emojis based on physiological detection could be only one option, and users could choose the one showing their real state, or others.

%Only one pair said they would like to see each other's EEG signals if there was such a feature. 
%When further being asked their reasons, they indicated that they were more interested in some hints that what the other is thinking about, not the signal itself. With the exception of this pair, no one else actively mentioned  the need for physiological signal visualization or interaction in the virtual environments for meditation. 
%When further asked about their reasons, they indicated that they were more interested in some hints about what the other was thinking about, not the signal itself. With the exception of this pair, no one else actively mentioned the need for physiological signal visualization or interaction in virtual environments for meditation.

\subsection{Privacy}
%When the experimenters asked the couples if you needed to add privacy features to the program, such as certain virtual objects that only you can see and not share with each other. 
When the experimenters asked the couples if they needed to add privacy features to the program, such as certain virtual objects that only an individual could see and not share with each other, the couples said no.
All said they did not need such a feature and that all content could be shared with each other. 
One participant looked at his partner and jokingly said, \textit{``Couples don't need privacy.'' - $C3_M$}


%\subsection{Design process}
%We found that couples' relationships are very private and personal during our meditation workshops. In the meditation experience phase in one workshop session involved two pairs, one pair intentionally chose to sit besides a pillar in the office so as to separate from the other pair in location and space. In addition, there were limited communication between couples in the design phase, even we encouraged them to communicate with each other. Interestingly, in one workshop session involved four people, who have known each other for some time before the workshop, they had limited communications between couples, too.   
%During our meditation workshops, we found that couples' relationships are very private and personal. In the meditation experience phase in one workshop session involving two pairs, one pair intentionally chose to sit beside a pillar in the office so as to separate from the other pair in location and space. In addition, there was limited communication between couples in the design phase, even though we encouraged them to communicate with each other. Interestingly, in one workshop session involving four people who had known each other for some time before the workshop, they had limited communication between couples, too.

%Couples' relationships are very private and personal, and we found during our meditation experience that in two workshops, two couples would purposely find a pillar to separate their two couples. This was not because they were unfamiliar with each other, as the four people attending one workshop knew each other well before the workshop. Also, during the design process, we found that each couple had little or no communication with each other, even after we strongly suggested that they communicate with each other.

%The design process is designed by the couple together and they contribute together. At the beginning, the couple planned together and will take into account the preferences and likes of both. Some make an outline and then draw it out together. 

%\begin{quote}
%    \textit{``We decided on this scene together, which is where we had our first date. I like music, so I drew a radio, and he really likes cartoon pillows, so he added this cute pillow to the scene.'' - $C6_F$}

    %\textit{``We barely communicated with them, I don't think they were able to suggest anything to our scene, and similarly we were, you know, these are our own memories. And I don't have their memories.'' - $C7_M$}
%\end{quote}

%Couples do not have a clear division of labor in the design process; 
%they decide on a general framework for the scene and then add details according to their own and their partners' preferences.
%instead, they settle on a broad framework for the scenario and then add elements based on their own and their partner's preferences.



==> Source/6-prototype-design.tex <==
\section{Feasibility Analysis}

Although we had some conclusions from the workshop, this still needed to be verified in VR. Therefore, we created a prototype based on the findings from the workshop and performed a feasibility analysis.


\subsection{Prototype design}
Based on our analysis and findings, we selected 5 design requirements to design our prototype.

    \begin{enumerate} 
        \item There are several meditation environments, one of which is the interior of a cozy house as a base. There is a pet in the room that can be interacted with by the user.
        \item There are multiple human-like avatars chosen by the user, including a couple avatar (the avatar's clothing and design are paired for men and women).
        \item The user's avatar can interact, and there will be special effects when making some special interactive movements, such as hand-holding, touching the head and body.
        \item Meditation guided voice and scene correlation and after the meditation starts the user will be fixed in a special place.
        \item Support remote login and voice communication.
    \end{enumerate}

The prototypical virtual space was made by Unity3D\footnote{\url{https://unity.com/}}, and we used Photon Engine\footnote{\url{https://doc.photonengine.com/en-us/pun/current/getting-started/pun-intro}} to achieve network connection and multi-user function. The materials used in the scene and Avatar model are purchased from the Unity Asset Store. The final program is packaged as APK files and imported into two Meta Quest 2\footnote{\url{https://store.facebook.com/quest/products/quest-2/}} headsets as VR head-mounted displays.

Our prototype provides six avatars for the user to choose from (see Figure~\ref{fig:demoScense} a)). Among them \textit{Female} and \textit{Male} are matched in terms of clothing and design style, in other words, couple avatars.

\begin{figure}[h]
  \centering
  \includegraphics[width=1\linewidth]{Figures/demo.png}
  \caption{A screenshot of the prototype's interface for selecting avatars and three meditation scenes. a) 6 avatars selection interface, all of them are humanoid; b) home scene, through the floor-to-ceiling windows users can see the sea and garden. The home has a double bed with a kitten lying on the TV stand at the end of the bed; c) lavender field scene with a large lavender field outside the cabin and two side by side lounge chairs which are facing the lavender field; d) Underwater scene, there will be small fish and jellyfish swimming after the program runs.}
  \Description{A screenshot of the prototype's interface for selecting avatars and three meditation scenes. a) 6 avatars selection interface, all of them are humanoid; b) home scene, through the floor-to-ceiling windows users can see the sea and garden. The home has a double bed with a kitten lying on the TV stand at the end of the bed; c) lavender field scene with a large lavender field outside the cabin and two side by side lounge chairs which are facing the lavender field; d) Underwater scene, there will be small fish and jellyfish swimming after the program runs.}
  \label{fig:demoScense}
\end{figure}

Based on the above design requirements, our prototype includes 3 scenes (Figure~\ref{fig:demoScense} b), c), d)). One is a home scene, one is is a lavender scene, and another an underwater scene. The underwater scene was chosen because it was the highest average score in the VR scene selection, and the lavender field was customized for one of the couples who experienced our prototype this time, and they showed their imaginary lavender field in their design work in the workshop.

The home scene is a bedroom with a full wall of floor-to-ceiling windows. Through the floor-to-ceiling windows you can see the small garden, the sea and the blue sky. The bed has a comfortable looking comforter and pillows. There is also a mirror on the wall, through which the user can see their avatar. there is a TV stand in front of the bed, on which a small cat is lying, when the user pets the cat, the cat will make a meow \textasciitilde ~meow \textasciitilde ~and will pose very enjoyable. The bedroom is connected to a small checkroom, where bathrobes and pajamas are hung. We added some white noise and leisurely footsteps to the background sound of the home scene. 

For the lavender field scene we designed a small cabin with two side-by-side loungers outside the cabin. The loungers face a large field of lavender, which will gently sway with the breeze, while a few light bird chirps will come from the distance. The background music of this scene we added the sound of wind, bird chirping and a little soft music.

Underwater scenes have jellyfish and small fish swimming, water plants swinging with the current, there are bubbles coming out of the cracks in the rocks. There is the sound of bubbles gurgling in the background.

When the user's avatar hands touch each other, the two hands clasped together will show a heart spinning effect, and when the user touches another user's head and body with the hands, there will be a short sparking particle effect (see Figure~\ref{fig:demoInteraction}). 

\begin{figure}[h]
  \centering
  \includegraphics[width=1\linewidth]{Figures/DemoInteraction.png}
  \caption{The interaction and effects in the prototype. a), b), c) show the interaction effects between avatars, where a) is the fireworks particle effect generated by the contact between avatar's hand and chest, b) is the fireworks particle effect generated by touching avatar's head with hand, c) is the love rotation effect generated by the contact between avatar's hand and hand. d) shows the interaction with the kitten with avatar's hand.}
  \Description{The interaction and effects in the prototype. a), b), c) show the interaction effects between avatars, where a) is the fireworks particle effect generated by the contact between avatar's hand and chest, b) is the fireworks particle effect generated by touching avatar's head with hand, c) is the love rotation effect generated by the contact between avatar's hand and hand. d) shows the interaction with the kitten with avatar's hand.}
  \label{fig:demoInteraction}
\end{figure}

After users press the `start meditation' button in the program, the home scene will fix the user's position on the bed and the lavender scene will fix the user on the lounge chair, and then play the meditation guide audio to start the meditation for about 10 minutes, the meditation audio will be adjusted accordingly according to different scenes. For example, the home scene will let the user look out of the window and feel the comfortable environment, while the lavender scene will let users to feel the wind, bird chirping and lavender waves. Also, the ocean scene will let users focus their attention on the sound of water, jellyfish and small fish, etc. The meditation guidance script was adapted to relate with each scene to create a multi-dimensional synchronizing experience by mentioned specific visual elements in the virtual environments. For example, the audio for the home scene said:

\begin{quote}
    \textit{``Please gently look around our shared home. No matter where we are, we have this common world to settle each other down. Take your time, scan each area, the plants outside the window, the warm sunlight, the soft pillows. Choose an area that you like, stop, and feel it.''}
\end{quote}

There are also words aiming at making the user feel the presence of the partner. For example, the audio said: 

\begin{quote}
    \textit{``Now, we want to bring this love to each other by looking gently at your partner, gazing at his silhouette, scanning its eyes, shoulders, arms, and palms in turn.''}
\end{quote}

\subsection{Study design}

After the prototype was completed, we invited participants to experience it and invited them to give feedback. This section describes the process and results in detail.

\subsubsection{Participants}

We invited two of the couples who had attended the workshop to experience our prototype ($C3$ \& $C5$). The rationale for selecting participants for the prototype experience from those who had attended the workshop was that: 1) they already had some familiarity with meditation and VR, and 2) the prototype was designed based on the results of the workshop, and they not only belonged to our target users but also participated in the design. These two couples were selected because 1) they were highly engaged throughout the workshop and generated many ideas, and 2) both had over a year of experience in long-distance relationships and fit our target demographic very well. 3) $C3$ was the only pair of participants invited to our workshop who had co-meditation experience.

\subsubsection{Prototype experience}

$C3$ and $C5$ came to the experimental venue to experience the prototype separately, in the same place as the workshop. Participants will first fill out questionnaires (see Section~\ref{sec:Quantitative}) as the baseline, next experience a 35-minute prototype, then fill the questionnaires again, at last, followed by a 15-minute semi-structured interview. $C5$ was only experienced once due to an unsuitable schedule, where $C3$ came to experience twice, and the second prototype experience had the same process except that participants only fill out the questionnaires after the meditation experience since their questionnaires before meditation in the first experience were the baseline. After communicating with participants, only $C5_F$ would like to be measured the skin conductance during meditation, and other participants expressed that the attached sensor would make them distracted. 

\subsubsection{Participants' feedback}
Participants' feedback was categorized according to the following themes: (1) the advantages and disadvantages of the prototype; (2) its feasibility as a remote meditation tool for couples; 

\textbf{Pros and Cons of the prototype:}

Among the three scenes of the prototype, all participants preferred the home scene, two couples gave a common reason is that home makes them feel warm and comfortable, and they are eager to have a home like this with their lover in the real world.

\textit{``The scene of this home is very similar to what we designed that day, with large floor-to-ceiling windows, curtains, a bed, and a yard...this is what our home looks like in our dreams, but unfortunately we can't afford such a house in real life. I feel very warm that I can have such a home with her in the virtual world.'' - $C5$}

\textit{``The scene of home is the most comfortable and detailed, it is like a real home, and it is an indoor environment that will make me feel more relaxed and have a more profound impact.'' - $C3$}

The researcher specifically asked $C3$ why the home scene felt better than the lavender scene, because the lavender scene was the scene they designed during the workshop. The reason $C3$ gave was that although the lady liked the lavender field, when it comes to the actual VR experience, the lavender field as an outdoor scene made them not feel safe enough, \textit{``I will always feel that there is some animal or something will suddenly appear, I will keep very alert'' - $C3$}, so they can not completely relax, but home will let them feel very safe.

$C3$ and $C5$ both said they liked the interaction design, including the interaction between the two Avatars and the interaction between the Avatar and the kitten. The male participant in the group of $C3$ said after the experience that he kept holding hands with the female participant and touched her head while meditating. \textit{``I will hold hands and watch the love heart keep spinning around, and also touch her head to see the pink effects floating out, I will feel relaxed, I will have the feeling that my girlfriend has also been staring at the love heart'' - $C3_M$}. At the same time, they all pointed out the following limitations: the avatar does not have expressions; the avatar design is not very appealing the way of interaction can be more abundant.

\textit{``With all due respect, Avatar is not very good-looking. And because it does not look like my girlfriend, the meditation voice will sometimes let me look at her and feel her body or something, I will feel very out of play.'' - $C5_M$}

\textit{``Avatar would be nice if it had expressions. The current avatar makes me feel like someone is with me, but I can hardly correspond this avatar to him. If it can't be the same as a real person, it's fine to design a face pinching system similar to the game, so we can design the avatar we want.'' - $C3_F$}

Couples 1 and 2 want a greater range of interactions with Avatars and kitties, and both couples expressed a desire for haptic experiences.

\textit{``It would be better if I could take my girlfriend's hand and stroll around the lavender field like in reality. Just now I wanted my girlfriend to come to me in the house, I had an urge to take her hand and pull her over, I wanted to pull her to run in the lavender field...but I couldn't feel the sensation of squeezing her hand.'' - $C3_M$}

\textbf{Feasibility as a remote couples meditation tool:}

Couple 1 only experienced the prototype once, and their response was that they would like to utilize VR together for an extended period of time while separated by a great distance, but not together to meditate with VR equipment in the same room. Because they thought they couldn't interact with one another when meditating, despite the fact that they regarded communication as crucial in close relationships. However, if VR meditation is utilized as a complement to other types of entertainment, such as VR games and VR films, they will also try it for long-distance romantic relationships. In addition, they demonstrated that if there were some fundamental aspects that would enable them to construct their own meditation scenarios in VR, they would like it more and find it to be more effective over time.

Couple 2 experienced the prototype twice, three days apart, and had experience meditating together before participating in our workshop. They said they would be willing to use such a VR meditation program for a long time.

\textit{``If the app was made more sophisticated, like avatar better looking...we would definitely want to use it for a long time. It is wonderful that we can use this app to feel each other together when we are in long distance and go where we want to go, it can turn what we imagine into reality.'' - $C3$}

They also said that they thought the interaction between avatars was the most important part of the VR meditation program after experiencing our prototype twice, because they feel that in reality they are also expressing their inner love by holding hands, hugging, kissing, touching, etc.

The experimenter also asked Couple 2 how they felt different between the two experiences, and they said that the first time they might feel very immersed due to the novelty of the meditation, which they had not experienced at all before, so they would be distracted by the interesting interactions inside. But the second time they thought the novelty would be lighter and they could focus more on the meditation itself.

The female participant of Couple 2 stated that the headset was heavy that the pressure pinched her cheeks. This is a significant aspect that ruins the immersion and contemplative atmosphere.

\subsubsection{Quantitative data}
\label{sec:Quantitative}

Apart from qualitative data, we also explored participants' feedback on personal emotions (I-PANAS-SF~\cite{Panas}), compassion (CMAS-self and CMAS-other~\cite{compassionscale}), experience of close relationships (ECR-S~\cite{closerelationship}) and skin conductance. The feedback was collected by psychological instruments and a bio-detection device (same as in the workshop). We acknowledge that, due to small sample size, it is suggested that the data in Table~\ref{tab:ECR-S-Quant} (Appendix) can only serve as a supplementary information for qualitative analysis and facilitating the discussion. 
We highlight two interesting observation from $C5$ and $C3$ as follows. 
First, the lower skin conductance level indicated the decrease of the sympathetic autonomic activity, which means a more relaxed status. This was consistent with their statements describing feeling comfortable and relaxed. 
For instance, $C5$ showed no obvious promotion or reduction in personal emotions, compassion, and experience of close relationships. $C5_F$ had a decrease in skin conductance level compared with the baseline (0.20$\mu$S vs. 0.13$\mu$S). 
Second, they are willing to use it for the long-term, with a feeling of companion. % and can feel accompanied. 
This can also be verified through quantitative analysis. For example, $C3$ results indicated that they had more positive emotions, stronger compassion intentions for couples and the distress tolerance for couples, and less attachment avoidance and attachment anxiety about their close relationships. 
%This may be related to the statement that Second, they are willing to use it for a long-term and can feel accompanied. 
%However, because our sample is small, these data are only used as a reference for qualitative analysis and the discussion, which can be viewed in the Appendix~\ref{appendices} for more information. 

==> Source/7-participant-evaluation-new.tex <==
\section{Prototype Evaluation}

After the prototype was completed, we invited another group of participants to experience it and give feedback. %This section describes the prototype evaluation process and results in detail.

\subsection{Participants}

We recruited 8 couple participants (n = 16, 8 male, 8 female) aged 21 - 32 ($M = 25.25$, $SD = 3.04$) from a social network, with a mean familiarity with the VR device of 2.90 ($SD = 1.28$, on a 5-point Likert scale), and all participants self-reported interest in LKM, with a mean familiarity with the meditation of 2.56 ($SD = 0.87$, on a 5-point Likert scale). All participants' visual acuity was normal or corrected to normal (using contact lenses or glasses). 

\subsection{Experiment design}

Each couple should experience LKM remotely twice, once utilizing VC for conventional remote LKM and once utilizing our VR LKM prototype, Figure~\ref{fig:teaser} shows the experiment setting. Both meditations lasted roughly 10 minutes. During the VC LKM, the experimenter assisted the participants in changing the virtual background of the VC to a dynamic background consistent with the virtual environment in the VR. Additionally, the meditation guidance audio used in the VC and VR conditions was the same, and the same white noise as in the VR virtual environment was added to ensure that other variables were as consistent as possible. The experimenter would direct the participants to sit in the most comfortable position in the chair and would inform them that they could close or open their eyes as they wished during the LKM, and that they were not required to constantly look at the camera (VC condition). As a baseline, participants were required to complete the questionnaire once prior to beginning the LKM, and then again following each LKM. After each LKM, participants will be asked to take a 10-minute break. The order of participants' experiences was disrupted using the Latin square.

\subsection{Psychological instruments}
\label{sec:questionnaire}
We used three psychological instruments to measure participants' changes in positive and negative emotions, compassion, and the experience of close relationships. Participants completed each scale three times, at the baseline, at the end of the first LKM (VC or VR), and at the end of the second LKM (VR or VC).

International Positive and Negative Affect Schedule Short Form (PANAS-Short) measured the positive and negative affect with 5 items, respectively, with a 5-point Likert scale for each item~\cite{Panas}. A higher score indicates more positive or negative affect, respectively. 

The compassion aspect was measured by Compassion Motivation and Action Scales (CMAS-self and CMAS-other)~\cite{compassionscale}. For both CMAS-self and CMAS-other, we deleted the items that measure the compassion actions since our study focuses on the short-term effect and the participants have no spare time to participate in a long-term study of understanding compassion. The remained items used a 7-point Likert scale. In CMAS-self, 5 items measure the compassion intention and 7 items measure the compassion distress. Higher scores indicate more self-compassion. In CMAS-other, 3 items measure the compassion intention and 3 items measure the compassion distress, with higher scores indicative of more compassion to others. In addition, we adapted words describing other people like \emph{``others''} and \emph{``people''} as \emph{``my partner''} in all items to better fit the close relationship context. 

The experience of close relationship was measured by Experience in Close Relationship Scale - Short Form (ECR-S)~\cite{closerelationship}, in which each item corresponds to a 7-point Likert scale. 6 items measure attachment avoidance, and 6 items measure attachment anxiety. People who score high on either or both of these dimensions are assumed to have an insecure adult attachment orientation. 


\subsection{Results}
The participants' prototype experience results are discussed in two parts: (1) quantitative data analysis (2) participants' feedback.

\subsubsection{Quantitative data}
Figure~\ref{fig:PrototypeResult} depicts the results of the questionnaires for the 16 participants before the LKM (baseline) and after the LKM (VC or VR condition).
\label{sec:Quantitative}
%\textbf{Psychological Scales}

\begin{figure}[h]
  \centering
  \includegraphics[width=1\linewidth]{Figures/PrototypeResult.png}
  \caption{Participants' scores on psychological instruments after Baseline, completion of VC LKM and completion of VR LKM. Participants' scores on the CMAS-Other scale after performing VR LKM were significantly higher than VC, the ECR-S scale in the VR condition also scored slightly better than the VC. ($P<.05$(*), $P<.01$(**), $P<.001$(***))}
  \label{fig:PrototypeResult}
\end{figure}

\textbf{PANAS-Short.} We compare the effect of VC and VR on Negative affect and Positive affect using a one-way repeated measures ANOVA.  The results showed that there was not a statistically significant difference in Negative effect between Baseline ($M = 7.438$, $SD = 2.828$), VC ($M = 8.063$, $SD = 2.435$) and VR ($M = 7.125$, $SD = 3.096$) conditions ($F(2, 30) = .828, p = .447$). However, we can see from the visualization that the average negative effect after participants completed VC LKM was slightly higher than Baseline. After examining the specific items of the PANAS-Short, we discovered that the \emph{Ashamed } item scores for Negative impact increased significantly, which will be discussed in Section~\ref{sec:Feedback}. The visualization of the results reveals a trend of slowly increasing Positive affect scores for the Baseline ($M = 12.125$, $SD = 3.243$), VC ($M = 12.313$, $SD = 3.572$), and VR ($M = 13.500$, $SD = 3.983$) conditions, but this trend is not statistically significant ($F(2, 30) = 1.108, p = .343$).

\textbf{CMAS-self.} One-way repeated measures ANOVA showed that the conditions significantly affect the \textit{self-compassion distress tolerance} subscale ($F(2, 30) = 15.405, p<.0001$), with Baseline ($M=22.875$, SD=$8.397$), VC ($M=28.563$, SD=$6.264$) and VR ($M=30.063$, SD=$6.923$), and the \textit{self-compassion intention} subscale ($F(2, 30) = 10.326, p < .0005$) with Baseline ($M=19.688$, SD=$3.683$), VC ($M=24.063$, SD=$3.151$) and VR ($M=23.000$, SD=$4.099$) of the CMAS-self. Post-hoc tests confirm that participants had significantly higher ($p<.01$) self-compassion distress tolerance scores after completing VC LKM than Baseline, and after VR LKM also had significantly higher ($p<.01$) self-compassion distress tolerance scores than Baseline, but there was no significant difference ($p=.059$) between VC and VR conditions. After VC LKM ($p<.01$) and VR LKM ($p<.05$), participants will have a significantly higher self-compassion intention than Baseline, but not significant compared to VC LKM and VR LKM ($p=.203$). 

\textbf{CMAS-other.} The CMAS-Other scale was analyzed in the same manner as the CMAS-Self. The results of the analyses revealed that the participants' intention to have compassion ($F(2, 30) = 10.175, p<.0005$) for their partner and their availability of tolerance ($F(2, 30) = 10.175, p<.0005$) when their partner was suffering were significantly affected by the LKM method. Post-hoc tests confirm that compared to Baseline ($M=10.813$, SD=$3.563$), participants' scores on the compassion distress tolerance subscale of the CMA-other increased significantly after VR LKM ($M=15.813$, SD=$2.562$, $p<.0005$), after VC LKM ($M=11.563$, SD=$3.881$) scores were slightly but not significantly higher ($p=.423$) than Baseline.  Scores on LKM using VR were significantly higher ($p<.01$) than VC. In addition to this, scores on the compassion intention subscale also increased significantly after VR LKM ($M=16.813$, SD=$1.870$, $p<.01$) compared to Baseline ($M=13.750$, SD=$2.436$), after VR LKM ($M=14.975$, SD=$2.729$) the scores slightly increase but not significant ($p=.092$), the effect of VR LKM was significantly better ($p<.05$) than VC.

\textbf{ECR-S.} As in the previous analyses, we did One-way repeated measures ANOVA for the attachment anxiety and attachment avoidance subscales separately, and the results showed that Baseline ($M=18.500$, SD=$7.737$), VC ($M=17.563$, SD=$7.155$), and VR ($M=15.063$, SD=$7.637$) have a significant effect ($F(2, 30) = 4.463, p<.05$) on the attachment anxiety scores, however, post hoc analysis did not reveal significant differences between the conditions. The values of the attachment avoidance subscales for Baseline ($M=13.813$, SD=$7.250$), VC ($M=12.250$, SD=$6.496$), and VR ($M=10.188$, SD=$4.370$) were significantly different ($F(2, 30) = 5.105, p<.05$). Post hoc analyses showed that participants' attachment avoidance values decreased significantly ($p<.05$) after performing VR LKM compared to Baseline.

\subsubsection{Participants' feedback}
\label{sec:Feedback}
At the end of the experiment, each couple was interviewed briefly, and their responses were categorized according to the following themes: (1) the benefits and drawbacks of utilizing VC and VR prototype for LKM (2) the viability of the prototype as a remote LKM tool for couples in specific scenarios.

\textbf{Advantages and Disadvantages}

All couples (n = 16) agreed that VR is preferable to VC for LKM in remote settings, and the vast majority (n = 12) of participants stated that VR is more immersive and enjoyable than VC, and that a more immersive environment would make them more immersed during LKM. In addition, because VR can make them feel as if they are with their partner, they can appreciate each other more during LKM. Some participants (n = 8) mentioned that, despite the fact that the avatar was not particularly attractive, they liked the interactive function of the avatar, and the special effects generated after avatar interaction made them more willing to interact, which was positive feedback, and such a feature was not present in VC. Moreover, two participants mentioned that LKM with VR is more beginner-friendly, and that they would be more likely to become distracted and lose focus when performing LKM with VC.

VC also has advantages over VR. Several participants (n = 6) mentioned that they felt facial expressions were important, and that they frequently required expressions to communicate. However, the avatar in VR lacks expressions, whereas in VC, the partner's expressions can be accurately viewed, and participants can perceive each other's emotions from the expressions. Nevertheless, an increasing number of couples (n = 10) believe that VC's ability to display each other's facial expressions will make them feel awkward and unnatural. And because VC can make them feel as though they are in a meeting or interview, it can cause them to experience some anxiety. This may explain our previous data analysis result, which revealed that, following VC LKM, the average negative emotions of participants increased, as opposed to the Baseline.

\textbf{Willingness to use prototypes}

In general, participants exhibited a great deal of enthusiasm for the VR LKM, and a few of them (n = 2) even expressed a desire to be long-term contributors to our project using this prototype. However, more participants (n = 10) hoped that if they used the prototype for an extended period of time, the virtual scenes could be customized, and they would like to create their own space or experience richer virtual scenes. Some couples (n = 4) also desired more realistic interactions, such as the incorporation of haptic feedback and avatar facial expressions.


==> Source/7-participant-evaluation.tex <==
\section{Prototype Evaluation}

After the prototype was completed, we invited participants to experience it and invited them to give feedback. This section describes the prototype evaluation process and results in detail.

\subsection{Participants}

We invited two of the couples who had attended the workshop to experience our prototype, to facilitate the discussion below, we label the two couples as Couple 1 and Couple 2.(Couple 1: Female 23 years, Male 23 years; Couple 2: Female 24 years, Male 25 years. All Eastern cultural background). The rationale for selecting participants for the prototype experience from those who had attended the workshop was that: 1) they already had some familiarity with meditation and VR, and 2) the prototype was designed based on the results of the workshop, and they not only belonged to our target users but also participated in the design. 
%These two couples were chosen because 1) they were very active during the workshop and came up with a lot of ideas, and 2) both of them had over one year of experience in long distance and were very well matched to our target demographic. 
These two couples were selected because 1) they were highly engaged throughout the workshop and generated many ideas, and 2) both had over a year of experience in long-distance relationships and fit our target demographic very well. 3) Couple 2 was the only pair of participants invited to our workshop who had co-meditation experience.

\subsection{Prototype experience}

Couple 1 and Couple 2 came to the experimental venue to experience the prototype separately, in the same place as the workshop. Participants will first fill out questionnaires (see Section~\ref{sec:Quantitative}) as the baseline, next experience a 35-minute prototype, then fill the questionnaires again, at last, followed by a 15-minute semi-structured interview. Couple 1 was only experienced once due to an unsuitable schedule, where Couple 2 came to experience twice, and the second prototype experience had the same process except that participants only fill out the questionnaires after the meditation experience since their questionnaires before meditation in the first experience were the baseline. After communicating with participants, only the female participant in Couple 1 would like to be measured the skin conductance during meditation, and other participants expressed that the attached sensor would make them distracted. 

\subsection{Results}
The results of the participants' prototype experience are discussed in two parts: (1) quantitative data analysis (2) participants' feedback.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}

\subsubsection{Quantitative data}
\label{sec:Quantitative}
\textbf{Psychological Scales}
We used three psychological instruments to measure participants' change in positive and negative emotions, compassion, and the experience of close relationships before and after the meditation experience. Couple 1 filled these psychological instruments for twice: before and after the meditation experience. Couple 2 filled for three times: before, after the first meditation experience, after the second meditation experience. 
%participants' sth... (change -> vague)
The positive and negative emotions was measured by International Positive and Negative Affect Schedule Short Form(I-PANAS-SF), which measured the positive and negative affect with 5 items respectively and the score range for both is 5 to 25 points , with a 5 point Liker-scale for each item (1 = not at all; 5 = Extremely)~\cite{Panas}. 

The compassion aspect was measured by Compassion Motivation and Action Scales (CMAS-self and CMAS-other)~\cite{compassionscale}. For both CMAS-self and CMAS-other, we deleted the items that measures the compassion actions since our study focus on the short-term effect and the participants have no spare time to participate a long-term study of understanding the compassion. The remained items used a 7 point Likert-scale from 1 to 7 (1 = strongly disagree, 7 = strongly agree). In CMAS-self, 5 items measure the compassion intention and 7 items measure the compassion distress so the score range is 5 to 35 and 7 to 49 respectively. In CMAS-other, 3 items measure the compassion intention and 3 items measure the compassion distress so the score range is 3 to 21 for both dimensions. In addition, we adapted words describing other people like \emph{``others''} and \emph{``people''} as \emph{``my partner''} in all items to better fit the close relationship context. 

The experience of close relationship was measured by Experience in Close Relationship Scale - Short Form (ECR-S)~\cite{closerelationship}, in which each item corresponds a 7 point Liker-scale (1 = strongly disagree, 7 = strongly agree). 6 items measure the attachment avoidance and 6 items measure the attachment anxiety so the score range for both is 6 to 42. 



% \begin{figure}[H]
%     \centering
%     \includegraphics[width=8cm]{Figures/PANAS.jpg}
%     \caption{Positive and negative affect change}
%     \label{fig:Positive and negative affect change}
% \end{figure}

%As the figure shows,
For Couple 1's response to I-PANAS-SF, the female participant had a slight increase in positive affect (17 vs. 19) and a decrease in negative affect (6 vs.5) after the meditation experience. The male participant only had a subtle decrease in negative affect(7 vs. 5). This implies that the meditation experience aroused participants' positive emotions and relieved negative emotions slightly. 
%Regarding to CMAS-self, the female participant remained the same respond, and the male participant had lightly increase in self-compassion intention(30 vs. 34) and self-compassion distress tolerance(35 vs. 36). 
In terms of CMAS-self, the female participant remained unchanged, while the male participant experienced a slight increase in self-compassion intention (30 vs. 34) and self-compassion distress tolerance (35 vs. 36).
%Regarding to CMAS-other, both of female and male participants didn't have obvious change in response before and after except the male participant had a very light increase in other-compassion distress tolerance (12 vs. 13). 
Regarding to CMAS-other, neither female nor male participants showed any discernible difference in response between before and after, with the exception of the male participant, who showed a very slight increase in other-compassion distress tolerance (15 vs. 16). 
As for the ECR-S, the female participant had a light decrease in attachment avoidance (25 vs. 23) and an increase in attachment anxiety (22 vs. 23). 
%The male participant had similar trend in terms of attachment avoidance (17 vs. 16) and attachment anxiety (18 vs. 19). 
Attachment avoidance (23 vs. 22) and attachment anxiety (24 vs. 25) were similar in the male participants.
Overall, the questionnaire response from Couple 1 was very subtle, with no obvious promotion or reduction in personal emotions, compassion, and experience of close relationships. 

For Couple 2, both female and male participants had an increase in positive affect (female: 16 vs. 18 vs. 19; male: 15 vs. 17 vs. 14) and a decrease in negative affect (female: 10 vs. 10 vs. 7; male: 15 vs. 8 vs. 7) in I-PANAS-SF. About CMAS, Couple 2 had a higher score in terms of self-compassion intention (female: 27 vs. 30 vs. 35; male: 23 vs. 33 vs. 35), self-compassion distress tolerance (female: 34 vs. 40 vs. 38 ; male: 35 vs. 43 vs. 40), other-compassion intention (female: 14 vs. 18 vs. 19; male: 20 vs. 21 vs. 20), other-compassion distress tolerance (female: 15 vs. 19 vs. 18; male: 20 vs. 21 vs. 19). 
The result indicated that Couple 2 had an improvement in compassion intention and distress tolerance for both individuals. %themselves and each other. 
In terms of ECR-S, the scores of both participants became roughly lower in attachment avoidance (female: 25 vs. 17 vs. 17; male: 12 vs. 9 vs. 15) and anxiety (female: 23 vs. 21 vs. 19; male: 29 vs. 19 vs. 18 ) after the meditation experience. 
Attachment avoidance means fear of dependence and interpersonal intimacy, and attachment anxiety means fear of interpersonal rejection or abandonment. Lower scores of attachment avoidance and anxiety imply a sense of security in intimacy relationships, and are negatively correlated with depression, anxiety, interpersonal distress, or loneliness. The result implies that the loving and kindness meditation experience was beneficial for participants' romantic relationships. 

\textbf{Bio-signal detection}
After seeking consent from the participants, we measured the skin conductance for the female participant in Couple 1 during the meditation experience. In addition, we measured for one minute as the baseline before the meditation started. The average skin conductance level in meditation sessions was lower than baseline (0.20$\mu$S vs. 0.13$\mu$S). The lower skin conductance level indicated the decrease of the sympathetic autonomic activity, that means a more relax status.  
%Apart from the psychological instruments, skin conductance change was recorded for the first visit of meditation experiences, containing a one-minute session (as a baseline), and three meditation sessions with breaks. 

\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%As shown in Figure~\ref{fig:xxx}, participants' negative effects decreased on the first and second day of meditation compared to before any meditation practice, while their positive effects remained rather consistent.

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=8cm]{Figures/Compassion.jpg}
%     \caption{Compassion Scale Change}
%     \label{fig:Compassion Scale Change}
% \end{figure}

%As the figure indicated, 
%The compassion intention and compassion tolerance increased after the first day of meditation and second day of meditation experience compared with the baseline status for both self-compassion and other compassion. However, there is no significant difference between the first day of meditation and the second day of meditation. This indicated that participants had a higher intent to be compassionate towards themselves and their romantic partner, with a higher ability to tolerate distress by themselves or their romantic partners when experiencing suffering. 

%\begin{figure}[H]
%    \centering
%    \includegraphics[width=8cm]{Figures/CloseRelationship.jpg}
%    \caption{Experience in close relationship scale result}
%    \label{fig:Experience in close relationship scale result}
%\end{figure}

%The last measured aspect is the Experience in Close Relationship, contains two sub-scales: attachment avoidance and attachment anxiety. Attachment avoidance means fear of dependence and interpersonal intimacy and attachment anxiety means fear of interpersonal rejection or abandonment. Higher scores of attachment avoidance and anxiety imply a sense of insecurity of intimacy relationship and positively correlated with depression, anxiety, interpersonal distress, or loneliness. %As the figure shows, 
%The score of attachment anxiety and attachment avoidance decreased compared with the baseline. This implies that the loving and kindness meditation experience was beneficial for participants' romantic relationships. 




% \begin{figure}[H]
%     \centering
%     \includegraphics[width=8cm]{Figures/figure of skin conductance.jpg}
%     \caption{Mean of Skin Conductance Level}
%     \label{fig:Mean of Skin Conductance Level}
% \end{figure}


\subsubsection{Participants' feedback}
Participants' feedback was categorized according to the following themes: (1) the advantages and disadvantages of the prototype (2) its feasibility as a remote meditation tool for couples.

\textbf{Pros and Cons of the prototype:}

Among the three scenes of the prototype, all participants preferred the home scene, two couples gave a common reason is that home makes them feel warm and comfortable, and they are eager to have a home like this with their lover in the real world.

\textit{Couple 1: ``The scene of this home is very similar to what we designed that day, with large floor-to-ceiling windows, curtains, a bed, and a yard...this is what our home looks like in our dreams, but unfortunately we can't afford such a house in real life. I feel very warm that I can have such a home with her in the virtual world.''}

\textit{Couple 2: ``The scene of home is the most comfortable and detailed, it is like a real home, and it is an indoor environment that will make me feel more relaxed and have a more profound impact.''}

The researcher specifically asked Couple 2 why the home scene felt better than the lavender scene, because the lavender scene was the scene they designed during the workshop. The reason Couple 2 gave was that although the lady liked the lavender field, when it comes to the actual VR experience, the lavender field as an outdoor scene made them not feel safe enough, \textit{``I will always feel that there is some animal or something will suddenly appear, I will keep very alert''}, so they can not completely relax, but home will let them feel very safe.

Couple 1 and Couple 2 both said they liked the interaction design, including the interaction between the two Avatars and the interaction between the Avatar and the kitten. The male participant in the group of Couple 2 said after the experience that he kept holding hands with the female participant and touched her head while meditating. \textit{``I will hold hands and watch the love heart keep spinning around, and also touch her head to see the pink effects floating out, I will feel relaxed, I will have the feeling that my girlfriend has also been staring at the love heart''}. At the same time, they all pointed out the following limitations: the avatar does not have expressions; the avatar design is not very appealing the way of interaction can be more abundant.

\textit{Couple 1: ``With all due respect, Avatar is not very good-looking. And because it does not look like my girlfriend, the meditation voice will sometimes let me look at her and feel her body or something, I will feel very out of play.''}

\textit{Couple 2: ``Avatar would be nice if it had expressions. The current avatar makes me feel like someone is with me, but I can hardly correspond this avatar to him. If it can't be the same as a real person, it's fine to design a face pinching system similar to the game, so we can design the avatar we want.''}

% Couple 1 and 2 both wanted more variety in the type of interaction with Avatars and kittens, and they both mentioned that they wanted have haptic sensations. 
Couples 1 and 2 want a greater range of interactions with Avatars and kitties, and both couples expressed a desire for haptic experiences.

\textit{Couple 2: ``It would be better if I could take my girlfriend's hand and stroll around the lavender field like in reality. Just now I wanted my girlfriend to come to me in the house, I had an urge to take her hand and pull her over, I wanted to pull her to run in the lavender field...but I couldn't feel the sensation of squeezing her hand.''}

\textbf{Feasibility as a remote couples meditation tool:}

% Couple 1 only experienced the prototype once, and the feedback they gave us was that they would want to use VR together for a long time when they were in a long distance, but not together for a long time to meditate with VR devices. Because they felt they couldn't communicate together while meditating, but they believed that communication was also very important in intimate relationships. However, if VR meditation is used as a supplement to other forms of entertainment such as VR games or VR movies, they would also try it when they are in a long distance. They also showed that if there were some basic elements that would then allow them to design their own meditation scenes in VR, they would enjoy it more and it would always be fresh and better for long-term use. 
Couple 1 only experienced the prototype once, and their response was that they would like to utilize VR together for an extended period of time while separated by a great distance, but not together to meditate with VR equipment in the same room. Because they thought they couldn't interact with one another when meditating, despite the fact that they regarded communication as crucial in close relationships. However, if VR meditation is utilized as a complement to other types of entertainment, such as VR games and VR films, they will also try it for long-distance romantic relationships. In addition, they demonstrated that if there were some fundamental aspects that would enable them to construct their own meditation scenarios in VR, they would like it more and find it to be more effective over time.

Couple 2 experienced the prototype twice, three days apart, and had experience meditating together before participating in our workshop. They said they would be willing to use such a VR meditation program for a long time.

\textit{Couple 2: ``If the app was made more sophisticated, like avatar better looking...we would definitely want to use it for a long time. It is wonderful that we can use this app to feel each other together when we are in long distance and go where we want to go, it can turn what we imagine into reality.''}

They also said that they thought the interaction between avatars was the most important part of the VR meditation program after experiencing our prototype twice, because they feel that in reality they are also expressing their inner love by holding hands, hugging, kissing, touching, etc.

The experimenter also asked Couple 2 how they felt different between the two experiences, and they said that the first time they might feel very immersed due to the novelty of the meditation, which they had not experienced at all before, so they would be distracted by the interesting interactions inside. But the second time they thought the novelty would be lighter and they could focus more on the meditation itself.

% The lady in Couple 2 reported that the headset was so heavy that it hurt her cheeks from the pressure. This is a major factor that ruins its immersion and meditative feel.
The female participant of Couple 2 stated that the headset was heavy that the pressure pinched her cheeks. This is a significant aspect that ruins the immersion and contemplative atmosphere.

==> Source/8-discussion.tex <==
\section{Discussion}

% explain our findings with related work and theories 
% design implications for love-kindness meditation in social VR for future designers and researchers

% 1. How doing love-kindness meditation in Social VR benefit remote romantic partners? 
% 1.1. summarize the benefits from our study
% 1.2 compare the benefits with the related work (e.g., Significant Otter, Bedtime Window etc.)
% highly social presence 
% avatar, exclusive environment to the partners 

% Design implication for doing love-kindness meditation in social VR
% key findings about the virtual environments and interactive objects, interaction methods 
% why some environments are more preferred than others? what are the potential reasons? 
% customized: how to customize the environment? 
%  shared experiences between the pair (personal value attached to it) psychology (endowment effect) 
% private: why they preferred a private environment instead of inviting pairs xxx 
% cite meditation work that allows multiple people to do so 
% multiple couples?? 

% abstract vs. concrete vs. 

% natural vs. indoor 

% animals: domestic vs. wild 

% interactive objects: 

% environmental psychology theory: human-made element (safe xxx) 

% enjoy an open view of the natural environment but also want to have a safe base 

% in traditional psychology, they studied the real objects; extends the theory to the VR environment. 
% as long as the environment complies with xxx characters, both realistic and xxx are possible 

% posture 
% face-to-face vs. facing the same direction (love-kindness meditation) 
% reasons xxx  (distraction: facial expressions may change or affect the thinking and meditation process) 
% benefit: enjoy the company of their partner; face-to-face creates pressure or distraction (cannot focus on meditation) 
% seeing facial expressions or biosignals may not be a positive thing (distraction, negative feedback): factors that cannot control may negatively affect them 
% design implications: 



% design process/thinking/rationale: 
% what role each participant played in the design
% collaborative design: 
% one designs the initial elements and gradually increase the element around the idea
% collaboratively design the initial elements 
% allow the partners to import personalized elements



Our participatory design method for VR meditation presents both opportunities and challenges for the design of VR remote meditation applications for couples while they are long-distance. In this section, we discuss each stage of the iterative design process and present reflections on the use of VR in social meditation for couples' relationships.

\subsection{Participatory design for couples}

Many studies of participatory design in which couples participate do not discuss the influence of the couple group on the process of participatory design~\cite{mcdonald2021building,lottridge2009sharing,chen2019draw}. However, we found some worthwhile discussions in the workshops for this study about couples engaging in participatory design.

In our workshops, couples rarely talk to each other, even if we strongly suggest they discuss it together. This was not because they were unfamiliar with each other, as all four people in two of the workshops were acquainted with each other. A reasonable explanation is that intimate relationships like couples are closed and introverted~\cite{bott2014family,cherlin1992marriage}, with a high degree of interdependence between partners~\cite{kalmijn2003shared}, this is also evidenced by the fact that couples actively choose the pillars in the conference room to separate them from each other when they meditate.

We observed during this workshop that there was a little discussion between different couples, and our topic did not necessarily require discussion between couples. Future researchers may consider a one-to-one format when conducting participatory designs for couples, i.e., one couple per session, rather than running a workshop format. If not required by the theme, the participation of multiple couples may only make it more difficult to organize and handle.

\subsection{Participatory design of meditation in VR}

Although previous studies have explored meditation in VR~\cite{patibanda2017life,prpa2018attending,roo2017inner}, no study has explored participatory design on this topic. So our workshop could only refer to previous participatory designs in VR themes and adapt them~\cite{flobak2019participatory,baker2019exploring}. The illustrated cards that we provided to participants in categories such as flowers, grass, water, animals, and weather were inspired by previous research~\cite{paredes2018driving,stepanova2020jel,roo2017inner,min2020effects}, however, we still found during the pilot study that the types of animals we prepared were not comprehensive and that perhaps pets would be more suitable for meditation. Our workshop showed that such card preparation is necessary, and the vast majority of participants (5/7) used the cards we prepared in their designs.

Participants' designs were not immediately presented to the participants in VR, which was not considered properly in this workshop, that's why when the lavender scene designed by Couple 2 is actually shown in VR to be realized, they don't feel as comfortable and relaxed as they thought. Future researchers could refer to Flobak et al.'s design~\cite{flobak2019participatory}, in which a technician could discuss with participants in real-time while they were designing meditation scenarios, and immediately implement some simple scenes and let participants experience them. Multiple iterations of the design would be more appropriate for such vague needs as meditation.

\subsection{Tailoring VR scenes for remote meditation for couples}

First of all, couples generally do not want to visualize physiological signals surprised us, many previous settings for meditation in VR visualized physiological data~\cite{patibanda2017life,prpa2018attending,stepanova2020jel,jarvela2021augmented,mevleviouglu2021visual,roo2017inner}. A possible reason for this is that negative emotions of partners in an intimate relationship may be passed on to each other~\cite{thompson1999emotional}, and several pairs of participants also noted that they did not want their partners to see their emotional changes.

Personalization is very important in remote VR couple meditation applications, including avatar customization and meditation scene customization. We suggest that future researchers could allow users to upload their own avatar photos to automatically generate a 3D avatar, or provide a face-pinching system that allows users to design their own avatar they want. For personalizing the meditation environment, it is possible to provide some basic elements, such as different indoor scenes, various furniture, and bonsai, different pets, etc., and let users build their desired home as a meditation environment together in the application.

The interaction between avatars is also important. In addition to the visual feedback when considering touching, hugging and holding hands, haptic feedback can also be considered. Nonverbal communication is an important part of intimacy~\cite{guerrero2006nonverbal}, and touch is the most intimate of the senses~\cite{andersen2008haptic}.

Finally, it is worth noting that the guided audio for meditation should correspond to the meditation environment, otherwise it will destroy the user's immersion and meditation experience.

%Limitation of the work 
%The demographic of the participants may impact the requirements collected in our study?

==> Source/9-conclusion.tex <==
\section{Conclusion}
This paper presents a participatory design approach to how long-distance couples can use VR as a tool for LKM to improve intimate relationships. In our study, we conducted a series of workshops to demonstrate participants' designs using our prepared materials and developed a remote VR couple meditation prototype based on the findings of the workshops. The results of couples experiencing the prototype were positive in personal emotions, compassion, close relationship experience, and willingness to long-term use.
%considered using VR for love and kindness meditation as a potential way to improve intimacy for long-distance couples. 

%Our participatory approach gives a series of design criteria for couples' VR meditation programs, and we hope that future program designers can build on our approach to design VR meditation applications suitable for couples and possibly include specific couples in the process of customizing virtual reality environments to help address the specific requirements of their relationships.
Our participatory approach gives a set of design criteria for VR meditation programs for couples. We hope that programmers and designers will be able to leverage our approach to make VR meditation applications that are good for couples, and possibly include specific couples in the process of customizing virtual reality environments to meet the needs of their relationships. 
